Localization with Sampling-Argmax

Soft-argmax operation is commonly adopted in detection-based methods to localize the target position in a differentiable manner. However, training the neural network with soft-argmax makes the shape of the probability map unconstrained. Consequently, the model lacks pixel-wise supervision through the map during training, leading to performance degradation. In this work, we propose sampling-argmax, a differentiable training method that imposes implicit constraints to the shape of the probability map by minimizing the expectation of the localization error. To approximate the expectation, we introduce a continuous formulation of the output distribution and develop a differentiable sampling process. The expectation can be approximated by calculating the average error of all samples drawn from the output distribution. We show that sampling-argmax can seamlessly replace the conventional soft-argmax operation on various localization tasks. Comprehensive experiments demonstrate the effectiveness and flexibility of the proposed method. Code is available at https://github.com/Jeff-sjtu/sampling-argmax

==> supp_sections/experiment.tex <==
\section{Correlation Testing}
\label{sec:corr}


\begin{table}[ht]
    \vspace{-5mm}
    \caption{Correlation testing on MTFL.}
    \label{tab:corr}
    \centering
    \begin{tabular}{lcc}
        \toprule
        Method & Corr. (Abs) &  Corr. (Rel) \\
        \midrule
        Soft & -0.261 & -0.270 \\
        Soft w/ V.R & -0.267 & -0.282 \\
        Soft w/ D.R & -0.263 & -0.279 \\
        \midrule
        Samp. Uni. & -0.263 & -0.276 \\
        Samp. Tri. & -0.278 & -0.301 \\
        Samp. Gau. & \textbf{-0.327} & \textbf{-0.355} \\
        \bottomrule
    \end{tabular}
\end{table}
